The Complexity of Switching and FACTS Maximum-Potential-Flow Problems

This papers considers the problem of maximizing the load that can be served by a power network. We use the commonly accepted Linear DC power network model and consider wo configuration options: switching lines and using FACTS devices. We present the first comprehensive complexity study of this optimization problem. Our results show hat the problem is NP-complete and that there is no fully polynomial-time approximation scheme. For switching, these results extend to planar networks with a aximum-node degree of 3. Additionally, we demonstrate that the optimization problems are still NP-hard if we restrict the network structure to cacti with a maximum degree of 3.

==> intro.tex <==
\section{Introduction}
In this paper we study the computational complexity of the maximum flow problem in electrical power systems for two types of reconfiguration options---\emph{switching} of lines (i.e., edges in the network) and utilizing \emph{flexible alternating current transmission system} (FACTS) devices---under the linear DC model.
Power systems exhibit the phenomenon \emph{Braess Paradox} \cite{Braess_1968_UbereinParadoxon}, whereby switching off lines can increase the maximum power flow.
This is because flows in power lines depend on the difference of potentials of the corresponding nodes. 
This creates cyclic dependencies that can be eliminated by switching.
The purpose of this research is to determine if there exists an efficient algorithm to solve these problems for real-world power networks.

Switching means physically disconnecting two nodes that were previously connected. 
The switching problem is to find a network configuration that allows for the maximum flow of power from the generators to the loads. 
On the other hand, FACTS allows us to change line parameters that would otherwise be fixed, e.g., susceptance. 
The FACTS problem is to find line parameter values that allow for the maximum flow of power from the generators to the loads. 
The difference between these two problems is that switching allows for a discrete choice whether or not the line is active, whereas FACTS allows the change of specific parameters of a line, where the parameter may take on any value between two given bounds.

Reconfiguring a network is necessary when parts of a network have failed, for example due to a disaster such as a cyclone, and the remaining network is not capable of satisfying the full demand.
\emph{Power restoration} is the problem of how, and in which order, the damaged power lines should be repaired to restore as much power as possible as fast as possible.  
It has been studied by power engineers for over 30 years (see \cite{adibi2000power} for a comprehensive collection of works). 
Besides finding the optimal sequence, more recent research also embeds the routing problem---repair crews need time to travel to the point of repair---into the optimization process \cite{PSCC11}.
As complementary research, we investigate the utilization of reconfiguration to improve the maximum power flow in the damaged network.
Reconfiguring the network can also be done as a first response on every step of the restoration.  
To the best of our knowledge, no complexity analysis has been done for this problem before.

In this paper, we present complexity results to answer the question: are there efficient algorithms to solve the switching and FACTS max flow problems? 
First we describe the problem in full mathematical detail (\cref{model}).
Then in \cref{sec:general_complexity}, we present general complexity results, which show that the problems cannot be approximated with a fully polynomial time approximation scheme.
Real power networks usually have a simple structure---they are almost planar and have a fixed maximum degree.
To be able to determine the complexity of real power networks, we worked on identifying the most ``complex'' networks structure where either problem is still polynomial.
In \cref{sec:beyond_trees} we show that \emph{cacti} with a fixed maximum degree of $3$ already make the problem NP-hard.
Additionally, we studied another simple relaxation of trees, called \emph{n-level Tree networks}, which are NP-hard to reconfigure as well.
This leads us to conclude that trees are the most ``complex'' network structure that is polynomial.
However, it might be possible to find a fully polynomial time approximation scheme for cacti and/or n-level tree networks.
We summarize our conclusions that we cannot expect to find a polynomial time algorithm to solve either of the switching or FACTS max flow configuration problems for real power networks in \cref{conclusion}.%
\footnote{The complexity results we present use unrealistic network parameters, but this is purely to obtain easy-to-handle proofs. 
The values can all be scaled to be realistic without influencing the results.}
Note that we only present the encodings of our complexity results; the proofs are given in appendix.
%A variety of optimization applications in electrical power systems involve on-the-fly reconfiguration and/or topology changes of the network.
%These include transmission planning \cite{BentAAAI}, vulnerability analysis \cite{Bienstock_2010_NkProblem}, power restoration \cite{PSCC11} and optimal power flow \cite{Fisher_2008_OptimalTransmissionSwitching}.
%
%Topology changes are achieved by \emph{switching} of power lines. 
%By switching lines we can exhibit \emph{Braess Paradox} \cite{Braess_1968_UbereinParadoxon}, the phenomenon by which removing (resp. adding) a line may increase (resp. decrease) the maximum possible power flow throughout the network. 
%Another way to influence power flows are \emph{Flexible Alternating Current Transmission System} (FACTS) devices.
%These allow the variation of otherwise fixed physical parameters of power lines.
%Utilising FACTS can help to deal with congestion and hence they can help improving the maximum possible power flow throughout the network.
%As of our knowledge, their is no systematic study based on theory of both optimization problems.
%
%In this paper we do a first study on the computational complexity of maximizing the power flow with respect to switching or the usage of FACTS devices.
%Our results show that in general the problem is NP-complete and there is no fully polynomial-time approximation scheme. 
%For switching this results extend to planar networks with a maximum-node degree of $3$.
%
%Power networks can not have arbitrary graph structures.
%They are usually planar and have a limited maximum degree.
%To know the complexity of both optimization problems for real world power system more precise, we worked on identifying the most complex networks structure where the problem is polynomial.
%Our voyage ended with trees as we discovered that \emph{cacti} with a fixed maximum degree of 3 are NP-hard.
%Although it might be possible to find an fully polynomial time approximation scheme.
%Additionally, we studied another simple relaxation of trees which called \emph{n-level Tree networks} which turned out to be NP-hard as well.
%
%Our complexity results are presented with network parameters that are unrealistic for real world networks.
%This is purely to obtain easy-to-handle proof.
%The values can all be scaled to be realistic without influencing the results.
%Hence, our results imply that we can not expect to find an algorithm that solves either optimization problem for real world power systems in polynomial time.
%
%The outline of the paper is as follows: in \cref{model} we present basic notations, the definitions and the flow models we use; \Cref{sec:general_complexity} presents the strongly NP-completeness results;
%\Cref{sec:beyond_trees} contains the results that cacti and n-level Tree networks are NP-hard and in \cref{conclusion} we draw conclusions and outline future work.
%Note that we only present the encodings of our complexity results.
%The proofs are omitted due to space reasons and can be found in the appendix.

